Creating Knowledge Graphs Subsets using Shape Expressions

The initial adoption of knowledge graphs by Google and later by big companies has increased their adoption and popularity. In this paper we present a formal model for three different types of knowledge graphs which we call RDF-based graphs, property graphs and wikibase graphs. In order to increase the quality of Knowledge Graphs, several approaches have appeared to describe and validate their contents. Shape Expressions (ShEx) has been proposed as concise language for RDF validation. We give a brief introduction to ShEx and present two extensions that can also be used to describe and validate property graphs (PShEx) and wikibase graphs (WShEx). One problem of knowledge graphs is the large amount of data they contain, which jeopardizes their practical application. In order to palliate this problem, one approach is to create subsets of those knowledge graphs for some domains. We propose the following approaches to generate those subsets: Entity-matching, simple matching, ShEx matching, ShEx plus Slurp and ShEx plus Pregel which are based on declaratively defining the subsets by either matching some content or by Shape Expressions. The last approach is based on a novel validation algorithm for ShEx based on the Pregel algorithm that can handle big data graphs and has been implemented on Apache Spark GraphX.

==> 50_ApplicationsKGSubsets.tex <==
\section{Use cases and Applications} \label{sec:Applications}

In this section we describe some use cases and applications were generating wikidata subsets is necessary.

\subsection{Scholia}

Scholia is a project that is based on 
 visualizing scientific information from Wikidata~\cite{Nielsen2017}\footnote{\url{https://scholia.toolforge.org/}}. 
 It offers visualizations about researcher's contributions which are currently generated from 
 direct SPARQL queries to the Wikidata Query Service. 

Given the size of Wikidata, visualizations that 
 need to are obtained from large number of results 
 can not be shown for several reasons:
\begin{itemize}
\item The queries require a lot of intermediate results which can not be manipulated
\item The complexity of the queries require more time than the 
 time slot provided by the wikidata query service. 
\item ...
\end{itemize}

As an example, the aspect that visualizes authors 
 by country only works for small countries. 

\todo[inline]{talk a bit more about this so we can later include experiment results...}

\subsection{GeneWiki project}

The GeneWiki project has been used as an running example with 
 domain-specific data to generate wikidata subsets in~\cite{LabraWikidataSubsetting21}. 

\todo[inline]{Talk more about this...compounds example?}

==> estructura.tex <==
\usepackage{pdfpages}

\DeclareUnicodeCharacter{20AC}{\euro{}} % to use euro 

\def\IEEET{IEEE Transactions}

\newcommand*{\formatfirst}[1]{\uppercase{#1}}
\newcommand*{\formatafter}[1]{\lowercase{#1}}
\makeatletter
\newcommand*{\mymacro}[1]{%
  \expandafter\formatfirst\expandafter{\@car #1\@empty\@nil}%
  \formatafter{\@cdr #1}\@empty\@nil}
\newcommand*\myMakeUpperCase[1]{%
  \def\@myuppercasewords{\expandafter\myuppercase@i#1 \@nil}%
    {\@myuppercasewords}\index{#1@\@myuppercasewords}}
\def\myuppercase@i#1 #2\@nil{%
  \mymacro{#1}%
  \ifx\\#2\\%
  \else
    \@ReturnAfterFi{%
      \space
      \myuppercase@i#2\@nil
    }%
  \fi
  }

\long\def\@ReturnAfterFi#1\fi{\fi#1}

\define@key{JCR}{autores}[default]{\def\JCR@autores{#1}}
\define@key{JCR}{titulo}[default]{\def\JCR@titulo{#1}}
\define@key{JCR}{clave}[default]{\def\JCR@clave{#1}}
\define@key{JCR}{nombre}[default]{\def\JCR@nombre{#1}}
\define@key{JCR}{numero}[default]{\def\JCR@numero{#1}}
\define@key{JCR}{paginas}[default]{\def\JCR@paginas{#1}}
\define@key{JCR}{editorial}[default]{\def\JCR@editorial{#1}}
\define@key{JCR}{ciudad}[default]{\def\JCR@ciudad{#1}}
\define@key{JCR}{pais}[default]{\def\JCR@pais{#1}}
\define@key{JCR}{fecha}[default]{\def\JCR@fecha{#1}}
\define@key{JCR}{issn}[default]{\def\JCR@issn{#1}}
\define@key{JCR}{index}[default]{\def\JCR@index{#1}}
\define@key{JCR}{anhoJCR}[default]{\def\JCR@anhoJCR{#1}}
\define@key{JCR}{impacto}[default]{\def\JCR@impacto{#1}}
\define@key{JCR}{posicion}[default]{\def\JCR@posicion{#1}}
\define@key{JCR}{tercil}[default]{\def\JCR@tercil{#1}}
\define@key{JCR}{categoria}[default]{\def\JCR@categoria{#1}}
\define@key{JCR}{otros}[default]{\def\JCR@otros{#1}}
\define@key{JCR}{cuartil}[default]{\def\JCR@cuartil{#1}}


\define@key{BOOK}{autores}[default]{\def\BOOK@autores{#1}}
\define@key{BOOK}{titulo}[default]{\def\BOOK@titulo{#1}}
\define@key{BOOK}{clave}[default]{\def\BOOK@clave{#1}}
\define@key{BOOK}{coleccion}[default]{\def\BOOK@coleccion{#1}}
\define@key{BOOK}{volumen}[default]{\def\BOOK@volumen{#1}}
\define@key{BOOK}{paginas}[default]{\def\BOOK@paginas{#1}}
\define@key{BOOK}{editorial}[default]{\def\BOOK@editorial{#1}}
\define@key{BOOK}{ciudad}[default]{\def\BOOK@ciudad{#1}}
\define@key{BOOK}{pais}[default]{\def\BOOK@pais{#1}}
\define@key{BOOK}{fecha}[default]{\def\BOOK@fecha{#1}}
\define@key{BOOK}{isbn}[default]{\def\BOOK@isbn{#1}}
\define@key{BOOK}{index}[default]{\def\BOOK@index{#1}}
\define@key{BOOK}{anhoBOOK}[default]{\def\BOOK@anhoBOOK{#1}}
\define@key{BOOK}{otros}[default]{\def\BOOK@otros{#1}}

\define@key{PROY}{titulo}[default]{\def\PROY@titulo{#1}}
\define@key{PROY}{efinanc}[default]{\def\PROY@efinanc{#1}}
\define@key{PROY}{referencia}[default]{\def\PROY@referencia{#1}}
\define@key{PROY}{convocatoria}[default]{\def\PROY@convocatoria{#1}}
\define@key{PROY}{entidades}[default]{\def\PROY@entidades{#1}}
\define@key{PROY}{duracion}[default]{\def\PROY@duracion{#1}}
\define@key{PROY}{ip}[default]{\def\PROY@ip{#1}}
\define@key{PROY}{ninv}[default]{\def\PROY@ninv{#1}}
\define@key{PROY}{responsabilidad}[default]{\def\PROY@responsabilidad{#1}}
\define@key{PROY}{publicaciones}[default]{\def\PROY@publicaciones{#1}}

\setkeys{JCR}{autores,titulo,clave,nombre,numero,paginas,editorial,ciudad,pais,fecha,issn,index,anhoJCR,impacto,posicion,tercil,categoria,otros}
\setkeys{BOOK}{autores,titulo,clave,coleccion,volumen,paginas,editorial,ciudad,pais,fecha,isbn,anhoBOOK,otros}
\setkeys{PROY}{titulo,efinanc,referencia,convocatoria,entidades,duracion,ip,ninv,responsabilidad,publicaciones}

\newcommand{\paper}[1]{
\setkeys{JCR}{autores,titulo,clave,nombre,numero,paginas,editorial,ciudad,pais,fecha,issn,index,anhoJCR,impacto,posicion,tercil,categoria,otros}%
\setkeys{JCR}{#1}%
\begin{flushleft}
\textbf{ Autores:} \JCR@autores \\
\textbf{ T\'itulo:} \JCR@titulo \\
\textbf{ Clave:} \JCR@clave \\
%\textbf{ Nombre de la revista:}  \myMakeUpperCase{\JCR@nombre} \\
\textbf{ Nombre de la revista:}  \JCR@nombre \\
\textbf{ N\'umero:} \JCR@numero \\
\textbf{ P\'aginas:} \JCR@paginas \\
\textbf{ Editorial:} \JCR@editorial \\
\ifthenelse{\equal{\JCR@ciudad}{default}}{}{\textbf{ Ciudad:} \JCR@ciudad \\}
\ifthenelse{\equal{\JCR@pais}{default}}{}{\textbf{ Pa\'is de publicaci\'on:} \JCR@pais \\}
\ifthenelse{\equal{\JCR@fecha}{default}}{}{\textbf{ A\~no de publicaci\'on:} \JCR@fecha \\}
\ifthenelse{\equal{\JCR@issn}{default}}{}{\textbf{ ISSN:} \JCR@issn \\}
\hspace{15mm}\framebox{
\begin{minipage}{12cm}
\textbf{ Indicios de calidad:} \\\small
\ifthenelse{\equal{\JCR@index}{default}}{}{{\em Base de datos de indexaci\'on:} \JCR@index\\}
\ifthenelse{\equal{\JCR@anhoJCR}{default}}{}{{\em A\~no de indexaci\'on:} \JCR@anhoJCR \\}
\ifthenelse{\equal{\JCR@categoria}{default}}{}{{\em Nombre de la categor\'ia:} \myMakeUpperCase{\JCR@categoria} \\}
\ifthenelse{\equal{\JCR@posicion}{default}}{}{{\em Posici\'on en la categor\'ia:} \JCR@posicion \\}
\ifthenelse{\equal{\JCR@impacto}{default}}{}{{\em Factor de impacto:} \JCR@impacto \\}
\ifthenelse{\equal{\JCR@tercil}{default}}{}{{\em Tercil:} \JCR@tercil \\}
\ifthenelse{\equal{\JCR@otros}{default}}{}{{\em Otros indicios:} \JCR@otros}
\end{minipage}
}
\end{flushleft}
}

\newcommand{\book}[1]{
\setkeys{BOOK}{autores,titulo,clave,coleccion,volumen,paginas,editorial,ciudad,pais,fecha,isbn,anhoBOOK,otros}%
\setkeys{BOOK}{#1}%
\begin{flushleft}
\textbf{ Autores:} \BOOK@autores \\
\textbf{ T\'itulo:} \BOOK@titulo \\
\textbf{ Clave:} Cap\'itulo de libro \\
\textbf{ Coleccion:}  \myMakeUpperCase{\BOOK@coleccion} \\
\textbf{ Volumen:} \BOOK@volumen\textbf{ P\'aginas:} \BOOK@paginas \\
\textbf{ Editorial:} \BOOK@editorial \\
\ifthenelse{\equal{\BOOK@ciudad}{default}}{}{\textbf{ Ciudad:} \BOOK@ciudad \\}
\ifthenelse{\equal{\BOOK@pais}{default}}{}{\textbf{ Pa\'is de publicaci\'on:} \BOOK@pais \\}
\ifthenelse{\equal{\BOOK@fecha}{default}}{}{\textbf{ A\~no de publicaci\'on:} \BOOK@fecha \\}
\ifthenelse{\equal{\BOOK@isbn}{default}}{}{\textbf{ ISSN:} \BOOK@isbn \\}
\hspace{5mm}\framebox{
\begin{minipage}{12cm}
\textbf{ Indicios de calidad:} \\\small
\ifthenelse{\equal{\BOOK@otros}{default}}{}{{\em Otros indicios:} \BOOK@otros}
\end{minipage}
}
\end{flushleft}
}


\newcommand{\proy}[1]{
\setkeys{PROY}{titulo,efinanc,referencia,convocatoria,entidades,duracion,ip,ninv,responsabilidad,publicaciones}%
\setkeys{PROY}{#1}%
\begin{flushleft}
\textbf{ T\'itulo del proyecto o contrato:} \PROY@titulo \\
\textbf{ Entidad financiadora:} \PROY@efinanc \\
\textbf{ Referencia del proyecto:} \PROY@referencia \\
\textbf{ Tipo de convocatoria:}  \PROY@convocatoria \\
\textbf{ Entidades participantes:} \PROY@entidades \\
\textbf{ Duraci\'on: } \PROY@duracion \\
\textbf{ Investigador principal:} \PROY@ip \\
\textbf{ N\'umero de investigadores: } \PROY@ninv \\
\textbf{ Aportaci\'on de la candidata al proyecto:} \PROY@responsabilidad \\
\ifthenelse{\equal{\PROY@publicaciones}{default}}{}{
\vspace{1mm}$ $\\\framebox{\begin{minipage}{12cm}\small
\textbf{ Justificaci\'on de la actividad investigadora en el contrato:} \\
\PROY@publicaciones
\end{minipage}
}
}

\end{flushleft}
}

\newcommand{\resalta}[1]{{\color{ocre} #1}}
\newcommand{\autores}[1]{\item[Autor(es):] #1}
\newcommand{\autor}[1]{\item[Autor:] #1}
\newcommand{\editores}[1]{\item[Editor(es):] #1}
\newcommand{\titulo}[1]{\item[Título:]{\resalta{#1}}}
\newcommand{\clave}[1]{\item[Clave:]#1}
\newcommand{\claveA}{\clave{Artículo}}
\newcommand{\claveP}{\clave{Preprint}}
\newcommand{\claveC}{\clave{Congreso}}
\newcommand{\nombreRevista}[1]{\item[Nombre revista:]#1}
\newcommand{\nombreCongreso}[1]{\item[Nombre congreso:]#1}
\newcommand{\referencia}[1]{\item[Referencia:]#1}
\newcommand{\institucion}[1]{\item[Institución:]#1}
\newcommand{\papel}[1]{\item[Papel:]#1}
\newcommand{\coordinador}[1]{\item[Coordinador:]#1}
\newcommand{\fecha}[1]{\item[Fecha:]#1}
\newcommand{\lugar}[1]{\item[Lugar:]#1}
\newcommand{\volumen}[1]{\item[Volumen:]#1}
\newcommand{\numero}[1]{\item[Número:]#1}
\newcommand{\pags}[1]{\item[Páginas:]#1}
\newcommand{\entidadFin}[1]{\item[Entidad financiadora:]#1}
\newcommand{\entidades}[1]{\item[Entidades participantes:]#1}
\newcommand{\duracion}[1]{\item[Duración:]#1}
\newcommand{\cuantia}[1]{\item[Cuantía de la subvención:]#1}
\newcommand{\participacion}[1]{\item[Participación:]#1}
\newcommand{\participantes}[1]{\item[Participantes:]#1}
\newcommand{\investigadores}[1]{\item[Investigadores:]#1}
\newcommand{\factorImpacto}[1]{\item[Factor de impacto:]#1}
\newcommand{\investPrincipal}[1]{\item[Investigador principal:]#1}

\newcommand{\doi}[1]{\item[doi:]\url{#1}}
\newcommand{\isbn}[1]{\item[ISBN:]#1}
\newcommand{\issn}[1]{\item[ISSN:]#1}

\newcommand{\urlProceedings}[1]{\item[URL:]\url{#1}}
\newcommand{\urlConferencia}[1]{\item[URL:]\url{#1}}
\newcommand{\urlVideo}[1]{\item[Video:]\url{#1}}
\newcommand{\urlCurso}[1]{\item[URL curso:]\url{#1}}

\newenvironment{jcr}{\begin{description}}{\vspace{0.2cm}\end{description}}

\newcommand{\curso}[1]{\item[Curso:]#1}
\newcommand{\internacional}{\item[Ámbito:]: Internacional}
\newcommand{\nacional}{\item[Ámbito:]: Nacional}

\newcommand{\editorial}[1]{\item[Editorial:]#1}
\newcommand{\GIISW}{Grado de Ing. Informática del Software}
\newcommand{\MIW}{Máster Univ. en Ingeniería Web}
\newcommand{\ASW}{Arquitectura del Software}
\newcommand{\WebSem}{Web Semántica}
\newcommand{\POO}{Programación Orientada a Objetos}
\newcommand{\NAWS}{Nuevos avances en Web Semántica}
\newcommand{\TICHA}{Tecnologías de la Información y la Comunicación para Historia del Arte}
\newcommand{\GHA}{Grado en Historia del Arte}
\newcommand{\LEW}{Lenguajes y estándares para la Web}
\newcommand{\ITIG}{Ingeniero Técnico en Informática de Gestión}
\newcommand{\ITIS}{Ingeniero Técnico en Informática de Sistemas}
\newcommand{\ITIGS}{Ingeniero Técnico en Informática de Gestión/Sistemas}
\newcommand{\II}{Ingeniero en Informática}
\newcommand{\coloreaFila}{\rowcolor{ocre!20}}

\newcommand{\mkdef}[1]{\index{#1}\emph{#1}}
\newcommand{\ingles}[1]{\emph{#1}}
% \newcommand{\indexn}[1]{\index{#1}#1}



==> myCommands.tex <==

\setcounter{secnumdepth}{2}	 
\setcounter{tocdepth}{3}	



%% Logic

\newcommand{\Limp}{\ensuremath{\rightarrow}}
\newcommand{\Lor}{\ensuremath{\vee}}
\newcommand{\Land}{\ensuremath{\wedge}}
\newcommand{\Lnot}{\ensuremath{\neg}}
\newcommand{\Ldimp}{\ensuremath{\leftrightarrow}}
\newcommand{\Lall}{\forall{}}
\newcommand{\Lexi}{\exists{}}
\newcommand{\Lder}{\ensuremath{\vdash{}}}
\newcommand{\Lraz}{\ensuremath{\vDash{}}}
\newcommand{\p}{\ensuremath{\varphi}}
\newcommand{\q}{\ensuremath{\psi}}

\newcommand{\LV}{\ensuremath{\mathbb{V}}}
\newcommand{\LF}{\ensuremath{\mathbb{F}}}

\newcommand{\mkdef}[1]{\index{#1}\emph{#1}}
\newcommand{\indexn}[1]{\index{#1}#1}
% \newcommand{\ingles}[1]{\emph{#1}}
\newcommand{\hazPeque}{\scriptsize}
\newcommand{\hazNormal}{\normalsize}
\newcommand{\resalta}{\textsl}

%
\newcommand{\Yandes}{\hspace{-0.5em}{\zap{}YANDES}}

% Colors

\definecolor{shadecolor}{rgb}{0.95,0.95,0.95}
\definecolor{cabTablaFondo}{rgb}{0,0.3,0}
\definecolor{cabTablaTxt}{rgb}{1,0.95,1}

\newenvironment{fuente}[1]
 {\begin{center}\begin{tabular}{|>{\scriptsize}m{1.6cm}|>{\scriptsize}m{10cm}|}
  \hline
  \multicolumn{2}{|m{11.6cm}|}{\small\bibentry{#1}} \\ 
  \hline
 }
 {\hline
  \end{tabular}\end{center}}



\newenvironment{programa}[2]
 {\begin{table}[H]
  \begin{tabular}{|>{\scriptsize}m{1.6cm}|>{\scriptsize}m{10cm}|}
  \hline
  \multicolumn{2}{|m{11.6cm}|}{#1 \newline {\scriptsize #2}} \\
  \hline
 }
 {\end{tabular}\end{table}}


\newenvironment{toc}
 {\begin{tocl}}
 {\end{tocl}}

\newenvironment{tocl}
  {\begin{list}{}
            {\setlength{\topsep}{-0.1em}
             \setlength{\itemsep}{-0.1em}}
  }
  {\end{list}}

\definecolor{letterColor}{rgb}{0,0.1,0}

%% First letter of chapter...
% \renewcommand{\LettrineFontHook}{\fontfamily{pzc}\fontshape{it}}

\newcommand{\letra}[2]{\lettrine[findent=0.2em,lhang=0.33,lines=2,loversize=0.2,lraise=0.2,slope=-.5em]
 {\color{letterColor}{#1}}{#2}}

% Arreglo temporal pq en mi despacho no tira el paquete calligra...
\newcommand{\calligra}{\zap}
\newcommand{\textcalligra}[1]{{\zap#1}}

\newenvironment{phrase}
 {\begin{quote}\calligra}{\end{quote}}

\newcommand{\txtph}[1]{{\hspace{-0.5em}\zap#1}}

\newsavebox{\quoteCiteBx}
\newenvironment{quoteCite}[1]
  {\begin{sloppypar}\begin{quote}\sbox{\quoteCiteBx}{\citep{#1}}\calligra}
  {\hspace*{\fill}\usebox{\quoteCiteBx}\end{quote}\end{sloppypar}}

\newsavebox{\quoteCHName}

\newenvironment{quoteCH}[1]
 {\begin{sloppypar}
  \begin{flushright}
    \begin{minipage}{9cm}\scriptsize\sffamily
      \sbox{\quoteCHName}{#1}
      \small\zap}
   {\hspace*{\fill}\usebox{\quoteCHName}\end{minipage}\end{flushright}\end{sloppypar}
    \vspace{2cm}
   }


%% Separaci�n en notaci�n BNF
\newcommand{\sep}{\,|\,}

\newcommand{\closeSemTab}{\ding{55}}

%% Contenido

\newcommand{\ponCreditos}[3]{
 {\scriptsize Cr�ditos:
  \ifthenelse{\equal{#1}{0}}{}{#1 Te.}
  \ifthenelse{\equal{#2}{0}}{}{#1 PT.}
  \ifthenelse{\equal{#3}{0}}{}{#3 PL.}
 }
}

\newenvironment{tema}[5]
 {\begin{table}[H]
  \begin{tabular}{|>{\scriptsize}m{1.6cm}|>{\scriptsize}m{10cm}|}
  \hline
  \multicolumn{2}{|m{11.6cm}|}{
     \begin{center}Tema #1. #2\end{center}
     \hfill \ponCreditos{#3}{#4}{#5}} \\ 
  \hline
 }
 {\end{tabular}
  \end{table}}

\newcommand{\TDC}[1]{Tabla de \newline{} Contenidos & #1 \\ \hline}
\newcommand{\COM}[1]{Comentarios & #1 \\ \hline}
\newcommand{\CONTENIDOS}[1]{Contenidos & #1 \\ \hline} 
\newcommand{\OBJETIVOS}[1]{Objetivos \newline específicos & #1 \\ \hline}
\newcommand{\SUGER}[1]{Sugerencias \newline pedagógicas & #1 \\ \hline}
\newcommand{\DESCRIPCION}[1]{Descripción & #1 \\ \hline}
\newcommand{\PREREQ}[1]{Pre-requisitos & #1 \\ \hline}
\newcommand{\BIBBAS}[1]{Bibliografía \newline B�sica & #1 \\ \hline}
\newcommand{\BIBCON}[1]{Bibliografía \newline de consulta & #1 \\ \hline}
\newcommand{\PRACTICAS}[1]{Prácticas & #1 \\ \hline}


\newenvironment{practica}[2]
 {\begin{table}[H]
  \begin{tabular}{|>{\scriptsize}m{1.6cm}|>{\scriptsize}m{10cm}|}
  \hline
  \multicolumn{2}{|m{11.6cm}|}{Práctica #1: #2} \\ 
  \hline
 }
 {\end{tabular}
  \end{table}}


\newenvironment{OBJ}
	{\begin{haskell}}
	{\end{haskell}}

\newcommand{\Osort}{\hskwd{sort}}
\newcommand{\Oop}{\hskwd{op}}
\newcommand{\Ois}{\hskwd{is}}
\newcommand{\Oobj}{\hskwd{obj}}
\newcommand{\Oendo}{\hskwd{endo}}
\newcommand{\Oeq}{\hskwd{eq}}
\newcommand{\Ocq}{\hskwd{cq}}
\newcommand{\Ovars}{\hskwd{vars}}
\newcommand{\Ovar}{\hskwd{var}}
\newcommand{\Osubsort}{\hskwd{subsort}}
\newcommand{\Oth}{\hskwd{th}}
\newcommand{\Oendth}{\hskwd{endth}}
\newcommand{\Oif}{\hskwd{if}}


%% Objetivos
\newcommand{\Ocon}{{\scriptsize\emph{(Conocimiento)}}}
\newcommand{\Ocom}{{\scriptsize\emph{(Comprensión)}}}
\newcommand{\Oapl}{{\scriptsize\emph{(Aplicación)}}}
\newcommand{\Oana}{{\scriptsize\emph{(Análisis)}}}
\newcommand{\Osin}{{\scriptsize\emph{(Síntesis)}}}
\newcommand{\Oeva}{{\scriptsize\emph{(Evaluación)}}}

\newcommand{\salto}{\vspace{0.6em}}

==> structure.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The Legrand Orange Book
% Structural Definitions File
% Version 2.1 (26/09/2018)
%
% Original author:
% Mathias Legrand (legrand.mathias@gmail.com) with modifications by:
% Vel (vel@latextemplates.com)
% 
% This file was downloaded from:
% http://www.LaTeXTemplates.com
%
% License:
% CC BY-NC-SA 3.0 (http://creativecommons.org/licenses/by-nc-sa/3.0/)
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%----------------------------------------------------------------------------------------
%	VARIOUS REQUIRED PACKAGES AND CONFIGURATIONS
%----------------------------------------------------------------------------------------

\usepackage{graphicx} % Required for including pictures
\graphicspath{{Pictures/}} % Specifies the directory where pictures are stored

% \usepackage{lipsum} % Inserts dummy text

\usepackage{tikz} % Required for drawing custom shapes

% \usepackage[english]{babel} % English language/hyphenation

\usepackage{enumitem} % Customize lists
\setlist{nolistsep} % Reduce spacing between bullet points and numbered lists

\usepackage{booktabs} % Required for nicer horizontal rules in tables

\usepackage{xcolor}

% \definecolor{ocre}{RGB}{243,102,25} % Define the orange color used for highlighting throughout the book
\definecolor{ocre}{RGB}{0,51,170}

%----------------------------------------------------------------------------------------
%	MARGINS
%----------------------------------------------------------------------------------------

\usepackage{geometry} % Required for adjusting page dimensions and margins

\geometry{
	paper=a4paper, % Paper size, change to letterpaper for US letter size
	top=3cm, % Top margin
	bottom=3cm, % Bottom margin
	left=3cm, % Left margin
	right=3cm, % Right margin
	headheight=14pt, % Header height
	footskip=1.4cm, % Space from the bottom margin to the baseline of the footer
	headsep=10pt, % Space from the top margin to the baseline of the header
	%showframe, % Uncomment to show how the type block is set on the page
}

%----------------------------------------------------------------------------------------
%	FONTS
%----------------------------------------------------------------------------------------

\usepackage{avant} % Use the Avantgarde font for headings
%\usepackage{times} % Use the Times font for headings
\usepackage{mathptmx} % Use the Adobe Times Roman as the default text font together with math symbols from the Sym­bol, Chancery and Com­puter Modern fonts

\usepackage{microtype} % Slightly tweak font spacing for aesthetics
\usepackage[utf8]{inputenc} % Required for including letters with accents
\usepackage[T1]{fontenc} % Use 8-bit encoding that has 256 glyphs

%--------------------------------------------------------------
%	BIBLIOGRAPHY AND INDEX
%--------------------------------------------------------------

\usepackage[
 style=numeric,
 citestyle=numeric,
 sorting=nyt,
 sortcites=true,
 autopunct=true,
 babel=hyphen,
 hyperref=true,
 abbreviate=false,
 backref=true,
 backend=biber]{biblatex}
 \addbibresource{knowledgeGraphs.bib} 

\defbibheading{bibempty}{}

\usepackage{calc} % For simpler calculation - used for spacing the index letter headings correctly
\usepackage{makeidx} % Required to make an index
\makeindex % Tells LaTeX to create the files required for indexing

%----------------------------------------------------------------------------------------
%	MAIN TABLE OF CONTENTS
%----------------------------------------------------------------------------------------

\usepackage{titletoc} % Required for manipulating the table of contents

\contentsmargin{0cm} % Removes the default margin

% Part text styling (this is mostly taken care of in the PART HEADINGS section of this file)
\titlecontents{part}
	[0cm] % Left indentation
	{\addvspace{20pt}\bfseries} % Spacing and font options for parts
	{}
	{}
	{}

% Chapter text styling
\titlecontents{chapter}
	[1.25cm] % Left indentation
	{\addvspace{12pt}\large\sffamily\bfseries} % Spacing and font options for chapters
	{\color{ocre!60}\contentslabel[\Large\thecontentslabel]{1.25cm}\color{ocre}} % Formatting of numbered sections of this type
	{\color{ocre}} % Formatting of numberless sections of this type
	{\color{ocre!60}\normalsize\;\titlerule*[.5pc]{.}\;\thecontentspage} % Formatting of the filler to the right of the heading and the page number

% Section text styling
\titlecontents{section}
	[1.25cm] % Left indentation
	{\addvspace{3pt}\sffamily\bfseries} % Spacing and font options for sections
	{\contentslabel[\thecontentslabel]{1.25cm}} % Formatting of numbered sections of this type
	{} % Formatting of numberless sections of this type
	{\hfill\color{black}\thecontentspage} % Formatting of the filler to the right of the heading and the page number

% Subsection text styling
\titlecontents{subsection}
	[1.25cm] % Left indentation
	{\addvspace{1pt}\sffamily\small} % Spacing and font options for subsections
	{\contentslabel[\thecontentslabel]{1.25cm}} % Formatting of numbered sections of this type
	{} % Formatting of numberless sections of this type
	{\ \titlerule*[.5pc]{.}\;\thecontentspage} % Formatting of the filler to the right of the heading and the page number

% Figure text styling
\titlecontents{figure}
	[1.25cm] % Left indentation
	{\addvspace{1pt}\sffamily\small} % Spacing and font options for figures
	{\thecontentslabel\hspace*{1em}} % Formatting of numbered sections of this type
	{} % Formatting of numberless sections of this type
	{\ \titlerule*[.5pc]{.}\;\thecontentspage} % Formatting of the filler to the right of the heading and the page number

% Table text styling
\titlecontents{table}
	[1.25cm] % Left indentation
	{\addvspace{1pt}\sffamily\small} % Spacing and font options for tables
	{\thecontentslabel\hspace*{1em}} % Formatting of numbered sections of this type
	{} % Formatting of numberless sections of this type
	{\ \titlerule*[.5pc]{.}\;\thecontentspage} % Formatting of the filler to the right of the heading and the page number

%----------------------------------------------------------------------------------------
%	MINI TABLE OF CONTENTS IN PART HEADS
%----------------------------------------------------------------------------------------

% Chapter text styling
\titlecontents{lchapter}
	[0em] % Left indentation
	{\addvspace{15pt}\large\sffamily\bfseries} % Spacing and font options for chapters
	{\color{ocre}\contentslabel[\Large\thecontentslabel]{1.25cm}\color{ocre}} % Chapter number
	{}  
	{\color{ocre}\normalsize\sffamily\bfseries\;\titlerule*[.5pc]{.}\;\thecontentspage} % Page number

% Section text styling
\titlecontents{lsection}
	[0em] % Left indentation
	{\sffamily\small} % Spacing and font options for sections
	{\contentslabel[\thecontentslabel]{1.25cm}} % Section number
	{}
	{}

% Subsection text styling (note these aren't shown by default, display them by searchings this file for tocdepth and reading the commented text)
\titlecontents{lsubsection}
	[.5em] % Left indentation
	{\sffamily\footnotesize} % Spacing and font options for subsections
	{\contentslabel[\thecontentslabel]{1.25cm}}
	{}
	{}

%----------------------------------------------------------------------------------------
%	HEADERS AND FOOTERS
%----------------------------------------------------------------------------------------

\usepackage{fancyhdr} % Required for header and footer configuration

\pagestyle{fancy} % Enable the custom headers and footers

\renewcommand{\chaptermark}[1]{\markboth{\sffamily\normalsize\bfseries\chaptername\ \thechapter.\ #1}{}} % Styling for the current chapter in the header
\renewcommand{\sectionmark}[1]{\markright{\sffamily\normalsize\thesection\hspace{5pt}#1}{}} % Styling for the current section in the header

\fancyhf{} % Clear default headers and footers
\fancyhead[LE,RO]{\sffamily\normalsize\thepage} % Styling for the page number in the header
\fancyhead[LO]{\rightmark} % Print the nearest section name on the left side of odd pages
\fancyhead[RE]{\leftmark} % Print the current chapter name on the right side of even pages
%\fancyfoot[C]{\thepage} % Uncomment to include a footer

\renewcommand{\headrulewidth}{0.5pt} % Thickness of the rule under the header

\fancypagestyle{plain}{% Style for when a plain pagestyle is specified
	\fancyhead{}\renewcommand{\headrulewidth}{0pt}%
}

% Removes the header from odd empty pages at the end of chapters
\makeatletter
\renewcommand{\cleardoublepage}{
\clearpage\ifodd\c@page\else
\hbox{}
\vspace*{\fill}
\thispagestyle{empty}
\newpage
\fi}

%----------------------------------------------------------------------------------------
%	THEOREM STYLES
%----------------------------------------------------------------------------------------

\usepackage{amsmath,amsfonts,amssymb,amsthm} % For math equations, theorems, symbols, etc

\newcommand{\intoo}[2]{\mathopen{]}#1\,;#2\mathclose{[}}
\newcommand{\ud}{\mathop{\mathrm{{}d}}\mathopen{}}
\newcommand{\intff}[2]{\mathopen{[}#1\,;#2\mathclose{]}}
\renewcommand{\qedsymbol}{$\blacksquare$}
\newtheorem{notation}{Notation}[chapter]

% Boxed/framed environments
\newtheoremstyle{ocrenumbox}% Theorem style name
{0pt}% Space above
{0pt}% Space below
{\normalfont}% Body font
{}% Indent amount
{\small\bf\sffamily\color{ocre}}% Theorem head font
{\;}% Punctuation after theorem head
{0.25em}% Space after theorem head
{\small\sffamily\color{ocre}\thmname{#1}\nobreakspace\thmnumber{\@ifnotempty{#1}{}\@upn{#2}}% Theorem text (e.g. Theorem 2.1)
\thmnote{\nobreakspace\the\thm@notefont\sffamily\bfseries\color{black}---\nobreakspace#3.}} % Optional theorem note

\newtheoremstyle{blacknumex}% Theorem style name
{5pt}% Space above
{5pt}% Space below
{\normalfont}% Body font
{} % Indent amount
{\small\bf\sffamily}% Theorem head font
{\;}% Punctuation after theorem head
{0.25em}% Space after theorem head
{\small\sffamily{\tiny\ensuremath{\blacksquare}}\nobreakspace\thmname{#1}\nobreakspace\thmnumber{\@ifnotempty{#1}{}\@upn{#2}}% Theorem text (e.g. Theorem 2.1)
\thmnote{\nobreakspace\the\thm@notefont\sffamily\bfseries---\nobreakspace#3.}}% Optional theorem note

\newtheoremstyle{blacknumbox} % Theorem style name
{0pt}% Space above
{0pt}% Space below
{\normalfont}% Body font
{}% Indent amount
{\small\bf\sffamily}% Theorem head font
{\;}% Punctuation after theorem head
{0.25em}% Space after theorem head
{\small\sffamily\thmname{#1}\nobreakspace\thmnumber{\@ifnotempty{#1}{}\@upn{#2}}% Theorem text (e.g. Theorem 2.1)
\thmnote{\nobreakspace\the\thm@notefont\sffamily\bfseries---\nobreakspace#3.}}% Optional theorem note

% Non-boxed/non-framed environments
\newtheoremstyle{ocrenum}% Theorem style name
{5pt}% Space above
{5pt}% Space below
{\normalfont}% Body font
{}% Indent amount
{\small\bf\sffamily\color{ocre}}% Theorem head font
{\;}% Punctuation after theorem head
{0.25em}% Space after theorem head
{\small\sffamily\color{ocre}\thmname{#1}\nobreakspace\thmnumber{\@ifnotempty{#1}{}\@upn{#2}}% Theorem text (e.g. Theorem 2.1)
\thmnote{\nobreakspace\the\thm@notefont\sffamily\bfseries\color{black}---\nobreakspace#3.}} % Optional theorem note
\makeatother

% Defines the theorem text style for each type of theorem to one of the three styles above
\newcounter{dummy} 
\numberwithin{dummy}{section}
\theoremstyle{ocrenumbox}
\newtheorem{theoremeT}[dummy]{Theorem}
\newtheorem{problem}{Problem}[chapter]
\newtheorem{exerciseT}{Exercise}[chapter]
\theoremstyle{blacknumex}
\newtheorem{exampleT}{Example}[chapter]
\theoremstyle{blacknumbox}
\newtheorem{vocabulary}{Vocabulary}[chapter]
\newtheorem{definitionT}{Definition}[section]
\newtheorem{corollaryT}[dummy]{Corollary}
\theoremstyle{ocrenum}
\newtheorem{proposition}[dummy]{Proposition}

%----------------------------------------------------------------------------------------
%	DEFINITION OF COLORED BOXES
%----------------------------------------------------------------------------------------

\RequirePackage[framemethod=default]{mdframed} % Required for creating the theorem, definition, exercise and corollary boxes

% Theorem box
\newmdenv[skipabove=7pt,
skipbelow=7pt,
backgroundcolor=black!5,
linecolor=ocre,
innerleftmargin=5pt,
innerrightmargin=5pt,
innertopmargin=5pt,
leftmargin=0cm,
rightmargin=0cm,
innerbottommargin=5pt]{tBox}

% Exercise box	  
\newmdenv[skipabove=7pt,
skipbelow=7pt,
rightline=false,
leftline=true,
topline=false,
bottomline=false,
backgroundcolor=ocre!10,
linecolor=ocre,
innerleftmargin=5pt,
innerrightmargin=5pt,
innertopmargin=5pt,
innerbottommargin=5pt,
leftmargin=0cm,
rightmargin=0cm,
linewidth=4pt]{eBox}	

% Definition box
\newmdenv[skipabove=7pt,
skipbelow=7pt,
rightline=false,
leftline=true,
topline=false,
bottomline=false,
linecolor=ocre,
innerleftmargin=5pt,
innerrightmargin=5pt,
innertopmargin=0pt,
leftmargin=0cm,
rightmargin=0cm,
linewidth=4pt,
innerbottommargin=0pt]{dBox}	

% Corollary box
\newmdenv[skipabove=7pt,
skipbelow=7pt,
rightline=false,
leftline=true,
topline=false,
bottomline=false,
linecolor=gray,
backgroundcolor=black!5,
innerleftmargin=5pt,
innerrightmargin=5pt,
innertopmargin=5pt,
leftmargin=0cm,
rightmargin=0cm,
linewidth=4pt,
innerbottommargin=5pt]{cBox}

% Creates an environment for each type of theorem and assigns it a theorem text style from the "Theorem Styles" section above and a colored box from above
\newenvironment{theorem}{\begin{tBox}\begin{theoremeT}}{\end{theoremeT}\end{tBox}}
\newenvironment{exercise}{\begin{eBox}\begin{exerciseT}}{\hfill{\color{ocre}\tiny\ensuremath{\blacksquare}}\end{exerciseT}\end{eBox}}				  
\newenvironment{definition}{\begin{dBox}\begin{definitionT}}{\end{definitionT}\end{dBox}}	
\newenvironment{example}{\begin{exampleT}}{\hfill{\tiny\ensuremath{\blacksquare}}\end{exampleT}}		
\newenvironment{corollary}{\begin{cBox}\begin{corollaryT}}{\end{corollaryT}\end{cBox}}	

%----------------------------------------------------------------------------------------
%	REMARK ENVIRONMENT
%----------------------------------------------------------------------------------------

\newenvironment{remark}{\par\vspace{10pt}\small % Vertical white space above the remark and smaller font size
\begin{list}{}{
\leftmargin=35pt % Indentation on the left
\rightmargin=25pt}\item\ignorespaces % Indentation on the right
\makebox[-2.5pt]{\begin{tikzpicture}[overlay]
\node[draw=ocre!60,line width=1pt,circle,fill=ocre!25,font=\sffamily\bfseries,inner sep=2pt,outer sep=0pt] at (-15pt,0pt){\textcolor{ocre}{R}};\end{tikzpicture}} % Orange R in a circle
\advance\baselineskip -1pt}{\end{list}\vskip5pt} % Tighter line spacing and white space after remark

%----------------------------------------------------------------------------------------
%	SECTION NUMBERING IN THE MARGIN
%----------------------------------------------------------------------------------------

\makeatletter
\renewcommand{\@seccntformat}[1]{\llap{\textcolor{ocre}{\csname the#1\endcsname}\hspace{1em}}}                    
\renewcommand{\section}{\@startsection{section}{1}{\z@}
{-4ex \@plus -1ex \@minus -.4ex}
{1ex \@plus.2ex }
{\normalfont\large\sffamily\bfseries}}
\renewcommand{\subsection}{\@startsection {subsection}{2}{\z@}
{-3ex \@plus -0.1ex \@minus -.4ex}
{0.5ex \@plus.2ex }
{\normalfont\sffamily\bfseries}}
\renewcommand{\subsubsection}{\@startsection {subsubsection}{3}{\z@}
{-2ex \@plus -0.1ex \@minus -.2ex}
{.2ex \@plus.2ex }
{\normalfont\small\sffamily\bfseries}}                        
\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}
{-2ex \@plus-.2ex \@minus .2ex}
{.1ex}
{\normalfont\small\sffamily\bfseries}}

%----------------------------------------------------------------------------------------
%	PART HEADINGS
%----------------------------------------------------------------------------------------

% Numbered part in the table of contents
\newcommand{\@mypartnumtocformat}[2]{%
	\setlength\fboxsep{0pt}%
	\noindent\colorbox{ocre!20}{\strut\parbox[c][.7cm]{\ecart}{\color{ocre!70}\Large\sffamily\bfseries\centering#1}}\hskip\esp\colorbox{ocre!40}{\strut\parbox[c][.7cm]{\linewidth-\ecart-\esp}{\Large\sffamily\centering#2}}%
}

% Unnumbered part in the table of contents
\newcommand{\@myparttocformat}[1]{%
	\setlength\fboxsep{0pt}%
	\noindent\colorbox{ocre!40}{\strut\parbox[c][.7cm]{\linewidth}{\Large\sffamily\centering#1}}%
}

\newlength\esp
\setlength\esp{4pt}
\newlength\ecart
\setlength\ecart{1.2cm-\esp}
\newcommand{\thepartimage}{}%
\newcommand{\partimage}[1]{\renewcommand{\thepartimage}{#1}}%
\def\@part[#1]#2{%
\ifnum \c@secnumdepth >-2\relax%
\refstepcounter{part}%
\addcontentsline{toc}{part}{\texorpdfstring{\protect\@mypartnumtocformat{\thepart}{#1}}{\partname~\thepart\ ---\ #1}}
\else%
\addcontentsline{toc}{part}{\texorpdfstring{\protect\@myparttocformat{#1}}{#1}}%
\fi%
\startcontents%
\markboth{}{}%
{\thispagestyle{empty}%
\begin{tikzpicture}[remember picture,overlay]%
\node at (current page.north west){\begin{tikzpicture}[remember picture,overlay]%	
\fill[ocre!20](0cm,0cm) rectangle (\paperwidth,-\paperheight);
\node[anchor=north] at (4cm,-3.25cm){\color{ocre!40}\fontsize{220}{100}\sffamily\bfseries\thepart}; 
\node[anchor=south east] at (\paperwidth-1cm,-\paperheight+1cm){\parbox[t][][t]{8.5cm}{
\printcontents{l}{0}{\setcounter{tocdepth}{0}}% The depth to which the Part mini table of contents displays headings; 0 for chapters only, 1 for chapters and sections and 2 for chapters, sections and subsections
}};
\node[anchor=north east] at (\paperwidth-1.5cm,-3.25cm){\parbox[t][][t]{15cm}{\strut\raggedleft\color{white}\fontsize{30}{30}\sffamily\bfseries#2}};
\end{tikzpicture}};
\end{tikzpicture}}%
\@endpart}
\def\@spart#1{%
\startcontents%
\phantomsection
{\thispagestyle{empty}%
\begin{tikzpicture}[remember picture,overlay]%
\node at (current page.north west){\begin{tikzpicture}[remember picture,overlay]%	
\fill[ocre!20](0cm,0cm) rectangle (\paperwidth,-\paperheight);
\node[anchor=north east] at (\paperwidth-1.5cm,-3.25cm){\parbox[t][][t]{15cm}{\strut\raggedleft\color{white}\fontsize{30}{30}\sffamily\bfseries#1}};
\end{tikzpicture}};
\end{tikzpicture}}
\addcontentsline{toc}{part}{\texorpdfstring{%
\setlength\fboxsep{0pt}%
\noindent\protect\colorbox{ocre!40}{\strut\protect\parbox[c][.7cm]{\linewidth}{\Large\sffamily\protect\centering #1\quad\mbox{}}}}{#1}}%
\@endpart}
\def\@endpart{\vfil\newpage
\if@twoside
\if@openright
\null
\thispagestyle{empty}%
\newpage
\fi
\fi
\if@tempswa
\twocolumn
\fi}

%----------------------------------------------------------------------------------------
%	CHAPTER HEADINGS
%----------------------------------------------------------------------------------------

% A switch to conditionally include a picture, implemented by Christian Hupfer
\newif\ifusechapterimage
\usechapterimagetrue
\newcommand{\thechapterimage}{}%
\newcommand{\chapterimage}[1]{\ifusechapterimage\renewcommand{\thechapterimage}{#1}\fi}%
\newcommand{\autodot}{.}
\def\@makechapterhead#1{%
{\parindent \z@ \raggedright \normalfont
\ifnum \c@secnumdepth >\m@ne
\if@mainmatter
\begin{tikzpicture}[remember picture,overlay]
\node at (current page.north west)
{\begin{tikzpicture}[remember picture,overlay]
\node[anchor=north west,inner sep=0pt] at (0,0) {\ifusechapterimage\includegraphics[width=\paperwidth]{\thechapterimage}\fi};
\draw[anchor=west] (\Gm@lmargin,-9cm) node [line width=2pt,rounded corners=15pt,draw=ocre,fill=white,fill opacity=0.5,inner sep=15pt]{\strut\makebox[22cm]{}};
\draw[anchor=west] (\Gm@lmargin+.3cm,-9cm) node {\huge\sffamily\bfseries\color{black}\thechapter\autodot~#1\strut};
\end{tikzpicture}};
\end{tikzpicture}
\else
\begin{tikzpicture}[remember picture,overlay]
\node at (current page.north west)
{\begin{tikzpicture}[remember picture,overlay]
\node[anchor=north west,inner sep=0pt] at (0,0) {\ifusechapterimage\includegraphics[width=\paperwidth]{\thechapterimage}\fi};
\draw[anchor=west] (\Gm@lmargin,-9cm) node [line width=2pt,rounded corners=15pt,draw=ocre,fill=white,fill opacity=0.5,inner sep=15pt]{\strut\makebox[22cm]{}};
\draw[anchor=west] (\Gm@lmargin+.3cm,-9cm) node {\huge\sffamily\bfseries\color{black}#1\strut};
\end{tikzpicture}};
\end{tikzpicture}
\fi\fi\par\vspace*{270\p@}}}

%-------------------------------------------

\def\@makeschapterhead#1{%
\begin{tikzpicture}[remember picture,overlay]
\node at (current page.north west)
{\begin{tikzpicture}[remember picture,overlay]
\node[anchor=north west,inner sep=0pt] at (0,0) {\ifusechapterimage\includegraphics[width=\paperwidth]{\thechapterimage}\fi};
\draw[anchor=west] (\Gm@lmargin,-9cm) node [line width=2pt,rounded corners=15pt,draw=ocre,fill=white,fill opacity=0.5,inner sep=15pt]{\strut\makebox[22cm]{}};
\draw[anchor=west] (\Gm@lmargin+.3cm,-9cm) node {\huge\sffamily\bfseries\color{black}#1\strut};
\end{tikzpicture}};
\end{tikzpicture}
\par\vspace*{270\p@}}
\makeatother

%----------------------------------------------------------------------------------------
%	LINKS
%----------------------------------------------------------------------------------------

\usepackage{hyperref}
\hypersetup{
  % hidelinks,
  backref=true,
  pagebackref=true,
  hyperindex=true,
% colorlinks=true,
  breaklinks=true,
%  urlcolor=ocre,
  bookmarks=true,
  bookmarksopen=false
}

\usepackage{bookmark}
\bookmarksetup{
open,
numbered,
addtohook={%
\ifnum\bookmarkget{level}=0 % chapter
\bookmarksetup{bold}%
\fi
\ifnum\bookmarkget{level}=-1 % part
\bookmarksetup{color=ocre,bold}%
\fi
}
}

